Real-time Level-of-Detail Strand-based Hair Rendering

Strand-based hair rendering has become increasingly popular in production for its realistic appearance. However, the prevailing level-of-detail solution employing hair cards for distant hair models introduces a significant discontinuity in dynamics and appearance during the transition from strands to cards. We introduce an innovative real-time framework for strand-based hair rendering that ensures seamless transitions between different levels of detail (LOD) while maintaining a consistent hair appearance. Our method uses elliptical thick hairs that contain multiple hair strands at each LOD to maintain the shapes of hair clusters. In addition to geometric fitting, we formulate an elliptical Bidirectional Curve Scattering Distribution Functions (BCSDF) model for a thick hair, accurately capturing single scattering and multiple scattering within the hair cluster, accommodating a spectrum from sparse to dense hair distributions. Our framework, tested on various hairstyles with dynamics as well as knits, shows that it can produce highly similar appearances to full hair geometries at different viewing distances with seamless LOD transitions, while achieving up to a 3x speedup.

==> Marschner.tex <==


\begin{figure}[hb]
\centering
\newcommand{\figcap}[1]{\begin{minipage}{0.46\linewidth}\centering#1\end{minipage}}
\hspace{0.04\linewidth}\hfill%
\figcap{Full w/ PT}\hfill%
\figcap{\textbf{LOD w/ ours}}\
\\
\hspace{0.04\linewidth}\hfill%
\includegraphics[trim={0   0   0   0  },clip,width=0.48\linewidth]{FIG/marschner_result/close_GT.png}\hfill%
\includegraphics[trim={0   0   0   0  },clip,width=0.48\linewidth]{FIG/marschner_result/close_ours.png}\hfill\\
\hspace{0.04\linewidth}\hfill%
\includegraphics[trim={370 370 370 370},clip,width=0.48\linewidth]{FIG/marschner_result/mid_GT.png}\hfill%
\includegraphics[trim={370 370 370 370},clip,width=0.48\linewidth]{FIG/marschner_result/mid_ours.png}\\
\hspace{0.04\linewidth}\hfill%
\includegraphics[trim={468 468 468 468},clip,width=0.48\linewidth]{FIG/marschner_result/far_GT.png}\hfill%
\includegraphics[trim={468 468 468 468},clip,width=0.48\linewidth]{FIG/marschner_result/far_ours.png}\\

\vspace{-39.2em}
\hspace{0.04\linewidth}\hfill%
\figcap{\color{white}{$1020$K triangles}}\hfill%
\figcap{\color{white}{$990$K triangles}}\\
\vspace{11.9em}
\hspace{0.04\linewidth}\hfill%
\figcap{\color{white}{$1020$K triangles}}\hfill%
\figcap{\color{white}{$713$K triangles}}\\
\vspace{11.9em}
\hspace{0.04\linewidth}\hfill%
\figcap{\color{white}{$1020$K triangles}}\hfill%
\figcap{\color{white}{$351$K triangles}}\\

\vspace{-24.5em}
\begin{flushleft}
{
\rotatebox{90}{Far view(2\%) \hspace{6em} Middle view(20\%) \hspace{6em}  Close view(60\%)   }\hfill%
}
\end{flushleft}

\vspace{3em}
\caption{While using \cite{MarschnerJCWH03} as single hair BCSDF, our strand-based LoD model(\textbf{LOD w/ ours}) effectively reduces the number of fibers and preserves appearance compared to path tracing with full hair geometry
(full w/ PT). And we mark the number of segments for hair strips in the image. }
%{\color{myRed}{Pink}} denotes the number of triangles for hair strips.}
\label{fig:marschner}
\Description{}
\end{figure}

==> bright_color.tex <==


\begin{figure}[hb]
\centering
\newcommand{\figcap}[1]{\begin{minipage}{0.46\linewidth}\centering#1\end{minipage}}
\hspace{0.04\linewidth}\hfill%
\figcap{Full w/ PT}\hfill%
\figcap{\textbf{LOD w/ ours}}\
\\
\hspace{0.04\linewidth}\hfill%
\includegraphics[trim={0   0   0   0  },clip,width=0.48\linewidth]{FIG/light_color_Result/close_GT.png}\hfill%
\includegraphics[trim={0   0   0   0  },clip,width=0.48\linewidth]{FIG/light_color_Result/close_ours.png}\hfill\\
\hspace{0.04\linewidth}\hfill%
\includegraphics[trim={370 370 370 370},clip,width=0.48\linewidth]{FIG/light_color_Result/mid_GT.png}\hfill%
\includegraphics[trim={370 370 370 370},clip,width=0.48\linewidth]{FIG/light_color_Result/mid_ours.png}\\
\hspace{0.04\linewidth}\hfill%
\includegraphics[trim={468 468 468 468},clip,width=0.48\linewidth]{FIG/light_color_Result/far_GT.png}\hfill%
\includegraphics[trim={468 468 468 468},clip,width=0.48\linewidth]{FIG/light_color_Result/far_ours.png}\\

\vspace{-39.2em}
\hspace{0.04\linewidth}\hfill%
\figcap{\color{red}{$1020$K triangles}}\hfill%
\figcap{\color{red}{$990$K triangles}}\\
\vspace{11.9em}
\hspace{0.04\linewidth}\hfill%
\figcap{\color{red}{$1020$K triangles}}\hfill%
\figcap{\color{red}{$713$K triangles}}\\
\vspace{11.9em}
\hspace{0.04\linewidth}\hfill%
\figcap{\color{red}{$1020$K triangles}}\hfill%
\figcap{\color{red}{$351$K triangles}}\\

\vspace{-24.5em}
\begin{flushleft}
{
\rotatebox{90}{Far view(2\%) \hspace{6em} Middle view(20\%) \hspace{6em}  Close view(60\%)   }\hfill%
}
\end{flushleft}

\vspace{3em}
\caption{Todo:}
\label{fig:brightcolor}
\Description{}
\end{figure}

==> largefigure.tex <==
\begin{figure*}[ht]
\centering
\newcommand{\figcap}[1]{\begin{minipage}{0.107\linewidth}\centering#1\end{minipage}}
\centering
\hspace{0.02\linewidth}\hfill%
\figcap{\small Near view}\hfill\figcap{\small Middle view}\hfill\figcap{\small Far view}\hfill
\figcap{\small Near view}\hfill\figcap{\small Middle view}\hfill\figcap{\small Far view}\hfill
\figcap{\small Near view}\hfill\figcap{\small Middle view}\hfill\figcap{\small Far view}\\
%\begin{flushleft}
%{\small \hspace{2.65em} Far view \hspace{2.35em} Middle view \hspace{1.9em} Near view
%\hspace{2.05em} Far view \hspace{2.35em} Middle view \hspace{1.9em} Near view
%\hspace{2.05em} Far view \hspace{2.35em} Middle view \hspace{1.9em} Near view
%}\end{flushleft}
\hspace{0.02\linewidth}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.107\linewidth]{FIG/Danielle/GT_0.png}\hfill%
\includegraphics[trim={320 320 320 320},clip,width=0.107\linewidth]{FIG/Danielle/GT_1.png}\hfill%
\includegraphics[trim={468 468 468 468},clip,width=0.107\linewidth]{FIG/Danielle/red_gt_2.png}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.107\linewidth]{FIG/Taro/GT_0.png}\hfill%
\includegraphics[trim={330 330 330 330},clip,width=0.107\linewidth]{FIG/Taro/GT_1.png}\hfill%
\includegraphics[trim={463 463 463 463},clip,width=0.107\linewidth]{FIG/Taro/blonde_gt_2.png}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.107\linewidth]{FIG/curly/GT_0.png}\hfill%
\includegraphics[trim={300 300 300 300},clip,width=0.107\linewidth]{FIG/curly/GT_1.png}\hfill%
\includegraphics[trim={463 463 463 463},clip,width=0.107\linewidth]{FIG/curly/GT_2.png}
\\
\vspace{-.3em}\hspace{0.02\linewidth}\hfill%
\figcap{\small (607K, --------)}\hfill\figcap{\small (607K, --------)}\hfill\figcap{\small (607K, --------)}\hfill
\figcap{\small (294K, --------)}\hfill\figcap{\small (294K, --------)}\hfill\figcap{\small (294K, --------)}\hfill
\figcap{\small (1,606K, --------)}\hfill\figcap{\small (1,606K, --------)}\hfill\figcap{\small (1,606K, --------)}\vspace{.4em}
\\
\hspace{0.02\linewidth}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.107\linewidth]{FIG/Danielle/ours_0.png}\hfill%
\includegraphics[trim={320 320 320 320},clip,width=0.107\linewidth]{FIG/Danielle/ours_1.png}\hfill%
\includegraphics[trim={468 468 468 468},clip,width=0.107\linewidth]{FIG/Danielle/ours_2.png}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.107\linewidth]{FIG/Taro/ours_0.png}\hfill%
\includegraphics[trim={330 330 330 330},clip,width=0.107\linewidth]{FIG/Taro/ours_1.png}\hfill%
\includegraphics[trim={463 463 463 463},clip,width=0.107\linewidth]{FIG/Taro/ours_2.png}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.107\linewidth]{FIG/curly/Ours_0.png}\hfill%
\includegraphics[trim={300 300 300 300},clip,width=0.107\linewidth]{FIG/curly/Ours_1.png}\hfill%
\includegraphics[trim={463 463 463 463},clip,width=0.107\linewidth]{FIG/curly/Ours_2.png}\vspace{-2.4em}
\\
\hspace{0.019\linewidth}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.04\linewidth]{FIG/Danielle/diff_ours_0.jpg}\hfill%
\includegraphics[trim={229 229 229 229},clip,width=0.04\linewidth]{FIG/Danielle/diff_ours_1.jpg}\hfill%
\includegraphics[trim={335 335 335 335},clip,width=0.04\linewidth]{FIG/Danielle/diff_ours_2.jpg}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.04\linewidth]{FIG/Taro/diff_ours_0.jpg}\hfill%
\includegraphics[trim={229 229 229 229},clip,width=0.04\linewidth]{FIG/Taro/diff_ours_1.jpg}\hfill%
\includegraphics[trim={335 335 335 335},clip,width=0.04\linewidth]{FIG/Taro/diff_ours_2.jpg}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.04\linewidth]{FIG/curly/diff_ours_0.jpg}\hfill%
\includegraphics[trim={229 229 229 229},clip,width=0.04\linewidth]{FIG/curly/diff_ours_1.jpg}\hfill%
\includegraphics[trim={335 335 335 335},clip,width=0.04\linewidth]{FIG/curly/diff_ours_2.jpg}
\\
\vspace{-.3em}\hspace{0.02\linewidth}\hfill%
\figcap{\small (514K, \textbf{66.66})}\hfill\figcap{\small (471K, \textbf{70.33})}\hfill\figcap{\small (197K, 73.69)}\hfill
\figcap{\small (231K, \textbf{67.24})}\hfill\figcap{\small (166K, \textbf{70.19})}\hfill\figcap{\small (\hspace{0.5em}83K, 72.57)}\hfill
\figcap{\small (1,306K, \textbf{64.02})}\hfill\figcap{\small (981K, \textbf{67.19})}\hfill\figcap{\small (197K, 66.23)}\vspace{.4em}
\\
\hspace{0.02\linewidth}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.107\linewidth]{FIG/Danielle/DS_0.png}\hfill%
\includegraphics[trim={320 320 320 320},clip,width=0.107\linewidth]{FIG/Danielle/DS_1.png}\hfill%
\includegraphics[trim={468 468 468 468},clip,width=0.107\linewidth]{FIG/Danielle/DS_2.png}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.107\linewidth]{FIG/Taro/DS_0.png}\hfill%
\includegraphics[trim={330 330 330 330},clip,width=0.107\linewidth]{FIG/Taro/DS_1.png}\hfill%
\includegraphics[trim={463 463 463 463},clip,width=0.107\linewidth]{FIG/Taro/DS_2.png}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.107\linewidth]{FIG/curly/DS_0.png}\hfill%
\includegraphics[trim={300 300 300 300},clip,width=0.107\linewidth]{FIG/curly/DS_1.png}\hfill%
\includegraphics[trim={463 463 463 463},clip,width=0.107\linewidth]{FIG/curly/DS_2.png}\vspace{-2.4em}
\\
\hspace{0.019\linewidth}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.04\linewidth]{FIG/Danielle/diff_DS_0.jpg}\hfill%
\includegraphics[trim={229 229 229 229},clip,width=0.04\linewidth]{FIG/Danielle/diff_DS_1.jpg}\hfill%
\includegraphics[trim={335 335 335 335},clip,width=0.04\linewidth]{FIG/Danielle/diff_DS_2.jpg}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.04\linewidth]{FIG/Taro/diff_DS_0.jpg}\hfill%
\includegraphics[trim={229 229 229 229},clip,width=0.04\linewidth]{FIG/Taro/diff_DS_1.jpg}\hfill%
\includegraphics[trim={335 335 335 335},clip,width=0.04\linewidth]{FIG/Taro/diff_DS_2.jpg}\hfill%
\includegraphics[trim={0 0 0 0},        clip,width=0.04\linewidth]{FIG/curly/diff_DS_0.jpg}\hfill%
\includegraphics[trim={229 229 229 229},clip,width=0.04\linewidth]{FIG/curly/diff_DS_1.jpg}\hfill%
\includegraphics[trim={335 335 335 335},clip,width=0.04\linewidth]{FIG/curly/diff_DS_2.jpg}
\\
\vspace{-.3em}\hspace{0.02\linewidth}\hfill%
\figcap{\small (607K,  63.30)}\hfill\figcap{\small (607K, 67.75)}\hfill\figcap{\small (607K, \textbf{74.28})}\hfill
\figcap{\small (294K, 64.05)}\hfill\figcap{\small (294K, 69.28)}\hfill\figcap{\small (294K, \textbf{75.33})}\hfill
\figcap{\small (1,606K, 62.04)}\hfill\figcap{\small (1,606K, 67.03)}\hfill\figcap{\small (1,606K, \textbf{74.38})}
\\
\vspace{-20.5em}
\begin{flushleft}{
\rotatebox{90}{\small \hspace{3.5em} DS \hspace{6.5em} \textbf{Ours} \hspace{6.5em} GT }\hfill%
}\end{flushleft}
\caption{\textbf{Hairstyles:} The ground truth (GT) and dual scattering (DS) are rendered with full hair geometry, while our approach utilizes reduced hair geometry with LoD. In contrast to DS, our results closely approximate the appearance of GT at close and middle views. While our approach exhibits some discrepancies around the silhouette resulting from the simplified hair geometry, these differences are less noticeable in practice, especially given the small screen occupancy (0.5\%). Additionally, our solution ensures a smooth transition between different LoDs. Notably, our method achieves a memory usage reduction of approximately 20\%, 35\%, and 70\% for near, middle, and far views, respectively, leading to an enhanced performance of up to $5\times$. The values in $(\bullet,\bullet)$ represent the number of hair segments and PSNR. The bottom right inset shows the error map, where brighter indicates a larger error.}
\label{fig:geometry_LOD}
\Description{}
\end{figure*}

==> lod.tex <==

%\subsection{Implementation details} %\label{sec:lodconstruction}



%We further extend their major and minor axis with a small user-defined parameter for 

%and compute their average position as the center $\cc^k = \sum_i \pp_i^k n_h$. 

%The decentralization matrix $\MM = [(\pp_1^k - \cc^k) ~ (\pp_2^k - \cc^k)~\cdots~(\pp_i^k - \cc^k) ]^T$

%\paragraph{Skinning weights computation}
%Skinning weights are computed based on

%\paragraph{Data structure}
%\kui{@tao, how we organize the hair strand data for LOD?}
%\textcolor{red}{Regarding the LOD hierarchy illustrated in the figure \ref{fig:LOD_Structre}, each cluster possesses its own hierarchical structure. The information for each level of LOD, where aggregated fibers are stored, includes details about multiple control planes. Each control plane encompasses the center's rest position, vectors describing the lengths and directions of major and minor axes, as well as interpolation data for simulation.}
%\begin{figure}[h]
%    \centering
%    \includegraphics[width=\linewidth]{FIG/LOD_structure.png}
%    \caption{Illustration of our LOD data structure }
%    \label{fig:LOD_Structre}
%\end{figure}

%\paragraph{Data update from simulation}
%During the construction of the LOD hierarchy, for each control point plane {center, $\rr$, $\rr$} of an aggregated fiber, we calculate and select three suitable positions and weights for simulation based on the position of the center. $\rr$ and $\rr$ undergo the same transformation as the triangle formed by the corresponding positions on the three guide hairs during the real-time motion.

%\kui{--------------}

%Primarily, due to the extremely large quantity of fibers, constructing LOD geometry structures dynamically for each frame incurs a time cost that real-time rendering cannot afford. Therefore, we choose to pre-process each assembly of filaments to determine its LOD geometry structure in advance, rather than performing this task in real time.

%For fabrics, that have an explicit hierarchical structure from fiber to ply, and then from ply to yarn, Zhao et al. \cite{Shuang16} proposed a method to compute procedural descriptions for fabric yarns. This can populate realistic fiber-level  details into yarn-based models, which also provide us with a three-tiered LOD (Level of Detail) structure. 

%However, the fibers in hair are relatively more free and independent from each other, which means we cannot employ the same method used for clothing to construct LOD. Therefore, we proposed a specific LOD construction method tailored for hair.
%After having the shading model for aggregated hair fiber, we need to propose a method to efficiently and accurately achieve real-time hair rendering. Unlike offline rendering, if we decide and perform suitable simplification from full hair for each frame, we first need to calculate the positions of each individual fiber and group them everytime before rendering. This incurs a considerable computational cost. Therefore, we propose a simulation-supported LOD structure based on the initial state of the hair. Firstly, we propose a method to fit a aggregated fiber as a tight bounding for a given cluster of hair. Then, we will provide a method for clustering individual hair fibers, aiming to enhance the efficiency of the LOD structure.

%\textbf{Aggregated Fiber Fitting}
%Giving a cluster of n hair fibers, we attempt to create a aggregated fiber, a frustum with a elliptical cross-section, to serve as a tight bounding for them. Solving this problem is inherently a challenging optimization task in three-dimensional space, and finding a relatively optimal solution can be time-consuming. Due to the large quantity of hair involved, the accuracy and precision from this optimization doesn't justify the additional time burden it incurs. Therefore, we simplifies the problem to multiple 2D plane optimizations, reducing time consumption. Firstly for each hair in this cluster, we obtain its k control points $c_{0}^i$, ... , $c_{k}^i$ with the same distance interval starting from root. The collection of the K-th control points for all hairs forms the input set for the K-th 2D plane optimizations we need. These points are termed $V_k := \{ c^1_k,c^2_k,c^3_k,...,c^n_k \}$. We aim to construct a cross-section of the aggregated fiber by this set of control points. For each set of control points $V_k$, we undergo a decentralization process on it, and treat the center $C_k$ as the ellipse's center. The decentralization data matrix M is 
%\begin{equation}
%M=
%\left[ \begin{array}{c}
%{(c^1_k - C_k)}^T\\
%{(c^2_k - C_k)}^T\\
%\vdots \\
%{(c^n_k - C_k)}^T\\
%\end{array} 
%\right ]
%\end{equation}

%Then we choose to use PCA (Principal Component Analysis) on this matrix to fit an ellipse for these points.
%\begin{equation}
%\frac{1}{n}M^TM = VS^2V^T
%\end{equation}
%We set the length of major axis $\gamma_A$ as $\sqrt{2} s1$, and the length of minor axis $\gamma_B$ as $\sqrt{2} s2$. The directions of the major and minor axes correspond to the respective eigenvector directions. After obtaining the ellipses fitted for each cross-section, our thick fiber will be formed by connecting these ellipse. The central axis of this frustum is the curve formed by connecting the centers of these ellipses. 

%\textbf{Filaments Clustering}
%Next, we need to start clustering the full hair to build the LOD structure. If we randomly choose hair for clustering, it will require a thicker aggregated fiber as the bounding for each cluster. This implies that at the same distance, we would need lower-level LOD for rendering for maintaining the appearance, reducing the efficiency gain from LOD. For this reason, we aim to cluster hairs that are close in Euclidean distance and do not exhibit significant differences in relative distance during the simulation. This goal aligns perfectly with the requirements of simulation. During animation, only several hundred hairs are selected as guide hairs for simulation, and the rest of the hairs have their movement guided by interpolating the displacement of three guide hairs. Hairs guided by the same set of guide hairs naturally meet our criteria. Inspired by \cite{Wang09}, 
%Therefore, we cluster hairs by their guide hairs and name these clusters as $Cluster_1, Cluster_2, ..., Cluster_m$. Fitting an aggregated hair fiber from the hairs in $cluster_i$ is the i-th primitive for our coarsest LOD level. And for lower LOD levels, since these hairs in a cluster are already guided by the same set of guide hairs, we need another approach for subdivision. Inspired by \cite{Wang09}, we adopt the metric to measure the difference between hairs and further subdivide $cluster_i$ into several smaller clusters.

\begin{comment}

\begin{algorithm}
    \caption{Aggregated Fiber Fitting}\label{lod_sudocode}
        \begin{algorithmic}[1]
%\Function{$Aggregated\_Fiber\_Fitting$}{cluster}
 \Function{$Fitting$}{cluster}
    \State $AggregatedFiber \gets \emptyset$
    \State $num\_p \gets $ the number of control points for a single hair
    \State $MAX\_LENGTH \gets$ the largest length of hairs 
    \State $interval \gets MAX\_LENGTH / (num\_p - 1)$ 
    \For{i=0 to $num\_p - 1$}
        \State $V_i \gets \emptyset$ 
        \For{hair in cluster}
            \State $V_i.PushBack(Get\_Points(hair, interval*i))$
        \EndFor
        \State $c_i \gets Center(V_i)$
        \State decentralized $V_i$ and save the data as a matrix M
        \State Perform PCA on M to obtain the major $\gamma_A$ and minor axes $\gamma_B$ of the cross-section.
        \State $CrossSection \gets \{c_i, \gamma_A, \gamma_B\}$
        \State $AggregatedFiber.PushBack(CrossSection)$
    \EndFor
    
    \Return AggregatedFiber
\EndFunction
        \end{algorithmic}
\end{algorithm}

\begin{algorithm}
    \caption{LOD Hierarchy Construction}\label{lod_sudocode}
        \begin{algorithmic}[1]
\Function{$LOD\_Build$}{cluster, n}
    \State $LOD\_level \gets ceil(\log_2n)$ 
    \State $num\_group \gets 1 $
    \State $LOD\_hierachy \gets \emptyset$
    \While{$LOD\_level>=0$}
        \State $groups \gets grouping(cluster, max(num\_group, n))$
        \State $layer \gets \emptyset$ 
        \For{i=1 to max(num\_group, n)}
            \State $aggregated\_fiber \gets Fitting$(groups[i])
            \State layer.PushBack($aggregated\_fiber$)
        \EndFor
        
        \State $LOD\_hierarchy.PushBack(layer)$
    \EndWhile
    \Return $LOD\_hierarchy$
\EndFunction
        \end{algorithmic}
\end{algorithm}



\subsection{Rendering(TBD)}\label{rendering}

\textbf{LOD Selection Strategy}

After obtaining LOD hierarchy, we also require an wise selection strategy that can minimize the number of primitives needed while ensuring no noticeable artifacts. We proposed a selection strategy primarily based on the following three components:

\begin{itemize}
    \item  
\textbf{density of thick fiber}
The hair density within a cluster significantly influences the choice of LOD level. When the hair density is low, such as a cluster formed by only a few relatively scattered flyaway fibers, using a single thick fiber to replace these hairs fills a substantial amount of the original free space. This discrepancy can lead to visible differences between the rendered result and the ground truth.

\item \textbf{width of thick fiber in screen space}
As most of the mainstream LOD techniques, the space occupied in screen space remains a crucial factor in LOD level selection. We limit the width of any fully visible line segment to be under 3 pixels. This limitation is applied because no matter how dense the hair within this thick hair, the fiber level details would be noticeably observed when exceeding 3 pixels width.

\item \textbf{visiblity of thick fiber}
For those thicker hairs situated more inward and closer to the head, they aren't entirely visible as a significant portion is obscured by several outer layers of hair. Increasing the LOD levels of this type of hair appropriately won't cause artifacts.
\end{itemize}
\end{comment}

==> lodcontructfig.tex <==


\begin{comment}\end{comment}
\begin{figure}[ht]
\centering
\includegraphics[trim={30 40 30 50},clip,width=\linewidth]{FIG/LoD.pdf}\vspace{-0.5em}
\begin{flushleft}{\footnotesize \hspace{0.em} (a) Single hairs \& LoD 0 \hspace{1.5em} (b) LoD 1 \hspace{3.5em} (c) LoD 2 \hspace{2.3em} (d) One hair cluster }\end{flushleft}
\caption{{Illustration of our LoD structure in 2D:} (a) 2048 single hairs (black dots) and $L_0$, (b) $L_1$, and (c) $L_2$. (d) is one hair cluster and its corresponding $L_{0,1,2}$ (red, green, and blue, respectively). Our fitting process only provides a rough approximated bounding ellipse for single hairs, and there is no bounding relation between $L_1$ to $L_{n_L-1}$. }
\label{fig:LoD_Structre}
\Description{}
\end{figure}  

==> scatterfig.tex <==

\begin{figure}[ht]
\centering
\newcommand{\figcap}[1]{\begin{minipage}{0.495\linewidth}\centering#1\end{minipage}}
\hspace{0.04\linewidth}\hfill%
\includegraphics[trim={40 22 40 40},clip,height=0.35\linewidth]{FIG/FIG_SIGA/scatteringPlot/azimuthal.png}\hfill%
\includegraphics[trim={40 22 40 40},clip,height=0.35\linewidth]{FIG/FIG_SIGA/scatteringPlot/longitudinal.png}\\
\vspace{-9em}
\begin{flushleft}{
\rotatebox{90}{\small \hspace{1em} {Scattering intensity} }\hfill%
}\end{flushleft}
\figcap{\small \hspace{2em} Azimuthal profile $\phi$ }\hfill%
\figcap{\small \hspace{0.5em} Longitudinal profile $\theta$ }\\
\caption{The average scattering intensity (green) across 100 ply instances with distinct fiber geometries. Our method (blue) offers a more accurate approximation than that of ~\cite{ZhuZJYA23} (orange), particularly in the azimuthal profile. }
\label{fig:scatterplot}
\Description{}
\end{figure}  
